Kinematic Modeling and Compliance Modulation of Redundant Manipulators Under Bracing Constraints

Collaborative robots should ideally use low torque actuators for passive safety reasons. However, some applications require these collaborative robots to reach deep into confined spaces while assisting a human operator in physically demanding tasks. In this paper, we consider the use of in-situ collaborative robots (ISCRs) that balance the conflicting demands of passive safety dictating low torque actuation and the need to reach into deep confined spaces. We consider the judicious use of bracing as a possible solution to these conflicting demands and present a modeling framework that takes into account the constrained kinematics and the effect of bracing on the end-effector compliance. We then define a redundancy resolution framework that minimizes the directional compliance of the end-effector while maximizing end-effector dexterity. Kinematic simulation results show that the redundancy resolution strategy successfully decreases compliance and improves kinematic conditioning while satisfying the constraints imposed by the bracing task. Applications of this modeling framework can support future research on the choice of bracing locations and support the formation of an admittance control framework for collaborative control of ISCRs under bracing constraints. Such robots can benefit workers in the future by reducing the physiological burdens that contribute to musculoskeletal injury.

==> README <==
              +---------------------------------------+
              |          THE IEEECONF CLASS           |
              | By Scott Pakin, scott+iecnf@pakin.org |
              +---------------------------------------+

Description
===========

The IEEEconf class implements the formatting dictated by the IEEE
Computer Society Press for conference proceedings
(ftp://pubftp.computer.org/press/outgoing/proceedings/instruct8.5x11.pdf).
IEEEconf.cls replaces latex8.sty and is compatible with any BibTeX
style, not just latex8.bst.  The goal was to produce a more faithful
implementation of the formatting rules and to do so with cleaner LaTeX
code than that provided by the latex8.* files.


Installation
============

Execute "latex IEEEconf.ins" to create IEEEconf.cls.  Install
IEEEconf.cls at an appropriate place in your directory tree (e.g., in
/usr/local/share/texmf/tex/latex/IEEEconf/ or
C:\localtexmf\tex\latex\IEEEconf\) and update the filename database,
if necessary.  See the UK TeX FAQ (http://www.tex.ac.uk/faq) for more
information on installing classes.

IEEEconf comes with prebuilt PDF documentation formatted for
U.S. Letter paper.  If you want to build the documentation from
scratch, the procedure is as follows:

    latex IEEEconf.dtx
    makeindex -s gind.ist IEEEconf
    makeindex -s gglo.ist IEEEconf.glo -o IEEEconf.gls
    latex IEEEconf.dtx


License
=======

Copyright (C) 2009 by Scott Pakin

This file may be distributed and/or modified under the conditions of
the LaTeX Project Public License, either version 1.3c of this license
or (at your option) any later version.  The latest version of this
license is in:

   http://www.latex-project.org/lppl.txt

and version 1.3c or later is part of all distributions of LaTeX
version 2006/05/20 or later.

